Visualizing a Moving Target: A Design Study on Task Parallel Programs in the Presence of Evolving Data and Concerns

Common pitfalls in visualization projects include lack of data availability and the domain users' needs and focus changing too rapidly for the design process to complete. While it is often prudent to avoid such projects, we argue it can be beneficial to engage them in some cases as the visualization process can help refine data collection, solving a "chicken and egg" problem of having the data and tools to analyze it. We found this to be the case in the domain of task parallel computing where such data and tooling is an open area of research. Despite these hurdles, we conducted a design study. Through a tightly-coupled iterative design process, we built Atria, a multi-view execution graph visualization to support performance analysis. Atria simplifies the initial representation of the execution graph by aggregating nodes as related to their line of code. We deployed Atria on multiple platforms, some requiring design alteration. We describe how we adapted the design study methodology to the "moving target" of both the data and the domain experts' concerns and how this movement kept both the visualization and programming project healthy. We reflect on our process and discuss what factors allow the project to be successful in the presence of changing data and user needs.

==> abstract.tex <==
% Place the contents of your abstract between the
% \begin{abstract} and \end{abstract} decorators.

\begin{abstract}

%Parallel and distributed programs orchestrate the cooperation of many computation resources to produce
%results that would be impossible to collect on a single machine. The complexity of orchestrating and
%fine-tuning the execution of these parallel and distributed computations requires careful consideration
%from the programmer.
%[Do we talk about AMT/ATR here at all?
%One such class of parallel runtimes is asynchronous task-based runtimes, which
%are unique from typical bulk-synchronous models. ]
%To optimize performance, the researchers need to examine how their back-end
%code is being executed.
% Through a tightly-coupled iterative design process, we built Atria,
%an execution tree visualization that allows the developers to examine causes of performance and to compare
%effects of different runtimes. We describe how throughout the design process, our visualization was a "moving target"
%and how this movement kept the both the visualization and programming project healthy. Our case study is an
%example of this dual benefit: how careful examination of a development version of Atria by the visualization experts
%lead to a discovery of a timing bug that prompted an in-depth discussion on collecting timing data by the
%performance and programming experts and lead to more careful design on both sides.
%To evaluate the efficacy of Atria, we conducted user studies with our collaborators and found that Atria
%provided an effective method of analyzing effects of changes in runtime policies.
%We reflect how our unique situation allowed us to not only follow the warnings against some common
%visualization design study pitfalls, but also to embrace certain pitfalls due to our circumstances.


Common pitfalls in visualization projects include lack of data availability and
  the domain users' needs and focus changing too rapidly for the design process
  to complete. While it is often prudent to avoid such projects, we argue it
  can be beneficial to engage them in some cases as the visualization process
  can help refine data collection, solving a "chicken and egg" problem of
  having the data and tools to analyze it. We found this to be the case in the
  domain of task-parallel computing.
%
  Parallel and distributed programs orchestrate the cooperation of many
  computation resources to produce results that would be impossible to collect
  on a single machine. The complexity of orchestrating and fine-tuning the
  execution of these parallel and distributed computations requires careful
  consideration from the programmer. However, few performance data collection
  and analysis tools are geared towards the specifics of task parallel
  paradigms. What changes need to be made are an open area of research.
%
 Despite these hurdles, we conducted a design study. Through a tightly-coupled
  iterative design process, we built Atria, a multi-view execution graph
  visualization to support performance analysis. Atria simplifies the initial
  representation of the execution graph by aggregating nodes as related to
  their line of code. We deployed Atria on multiple platforms, some requiring
  design alteration. Our evaluation is augmented with user interviews.
%
  We further describe how we adapted the design study methodology to the
  "moving target" of both the data and the domain experts' concerns and how
  this movement kept both the visualization and programming project healthy.
  We reflect on our process and discuss what factors allow the project to be
  successful in the presence of changing data and user needs.


%Common pitfalls in visualization design studies include lack of data
%availability and the domain users' needs and focus changing too rapidly for the
%design process to complete. While it is often prudent to avoid such projects, we
%argue it can be beneficial to engage them in some cases as the visualization
%process can help refine data collection, solving a ``chicken and egg'' problem
%of having the data and tools to analyze it. In this paper, we describe how we
%adapted design study methodology to the domain of task parallel computing -- a
%prime example of this kind of moving target. In this instance, we show how a
%tightly-coupled iterative design process kept both the visualization and the
%programming project healthy. We reflect on our process and discuss what factors
%allow the project to be successful in the presence of changing data and user
%needs.

%Parallel and distributed programs orchestrate the cooperation of many
%computation resources to produce results that would be impossible to collect on
%a single machine. The complexity of orchestrating and fine-tuning the execution
%of these parallel and distributed computations requires careful consideration
%from the programmer. However, few performance data collection and analysis tools
%are geared towards the specifics of task parallel paradigms. We present Atria, a
%multi-view execution graph visualization to support performance analysis. Atria
%simplifies the initial representation of the execution graph by aggregating
%nodes as related to their line of code. The evolution of its design, and its
%deployments in a variety of contexts, reveal key insights into open areas of
%research in task parallel computing.






\end{abstract}


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

